Preserving Plasticity in Continual Learning with Adaptive Linearity Injection

Loss of plasticity in deep neural networks is the gradual reduction in a model's capacity to incrementally learn and has been identified as a key obstacle to learning in non-stationary problem settings. Recent work has shown that deep linear networks tend to be resilient towards loss of plasticity. Motivated by this observation, we propose Adaptive Linearization (AdaLin), a general approach that dynamically adapts each neuron's activation function to mitigate plasticity loss. Unlike prior methods that rely on regularization or periodic resets, AdaLin equips every neuron with a learnable parameter and a gating mechanism that injects linearity into the activation function based on its gradient flow. This adaptive modulation ensures sufficient gradient signal and sustains continual learning without introducing additional hyperparameters or requiring explicit task boundaries. When used with conventional activation functions like ReLU, Tanh, and GeLU, we demonstrate that AdaLin can significantly improve performance on standard benchmarks, including Random Label and Permuted MNIST, Random Label and Shuffled CIFAR-10, and Class-Split CIFAR-100. Furthermore, its efficacy is shown in more complex scenarios, such as class-incremental learning on CIFAR-100 with a ResNet-18 backbone, and in mitigating plasticity loss in off-policy reinforcement learning agents. We perform a systematic set of ablations that show that neuron-level adaptation is crucial for good performance and analyze a number of metrics in the network that might be correlated to loss of plasticity.

==> sections/2-related_work.tex <==
\section{Related Work}
% \subsection{Loss of Plasticity in Deep Neural Networks}
Loss of plasticity in neural networks refers to the gradual decline in a model’s ability to learn and adapt to new data over time, a phenomenon that is particularly problematic in nonstationary learning settings such as continual learning and reinforcement learning~\citep{lyle2023understanding,dohare2024loss,nikishin2023deep}. As networks undergo prolonged training, they often become resistant to updates, limiting their capacity to integrate new information effectively. In recent years, various approaches have been proposed to mitigate this issue, broadly focusing on two aspects: (1) ensuring the network remains receptive to learning throughout training, and (2) improving generalization, preserving adaptability while also maintaining performance on unseen data~\citep{lee2024slow}. In this work, we validate our approach by analyzing its effectiveness in preserving both trainability (ensuring the network continues to perform well during training) while also monitoring its performance on test data for generalization.

To mitigate plasticity loss, several methods have been proposed in the last few years. Some focus on regularizing the network to retain properties beneficial for maintaining plasticity, such as preserving the initial task’s weights~\citep{kumar2023maintaining}, weight distribution~\citep{lewandowski2023curvature}, or structural characteristics of the weight matirx like orthogonality~\citep{chung2025parseval}. Others aim to restore learning capacity by identifying and reinitializing specific weights or neurons, either randomly or based on metrics like dormancy~\citep{dohare2024loss}. Finally, some approaches introduce architectural modifications, such as adding a secondary network~\citep{lee2024slow} or altering activation functions~\citep{abbas2023loss,lewandowski2024plastic}. Since our work centers on designing an adaptive activation function, we survey this research direction in detail. 

% next explore existing activation functions and their impact on maintaining plasticity.


% \subsection{Activation Functions in Loss of Plasticity}

% More recently, a number of studies have explored the effects of activation functions on plasticity and have proposed new designs to address its degradation. 

\citet{abbas2023loss} highlighted how standard ReLU activations contribute to activation collapse, leading to diminishing gradients and reduced learning capability in continual reinforcement learning. To counteract this, they introduced Concatenated ReLUs (CReLUs), which maintain activation diversity by duplicating activations with opposite signs, effectively ensuring that some portion of each neuron's output stays unsaturated. Their work underscores the critical role of activation function design in ensuring continual learning effectiveness in non-stationary environments. 

In \cite{lewandowski2024plastic}, the authors have demonstrated that linear networks exhibit resilience to loss of plasticity. This resilience applies to both simple linear function approximators and deep linear networks, which maintain stable training dynamics across sequential tasks. 
Building on this insight, they introduce deep Fourier features, an innovative architectural modification that incorporates fixed sinusoidal activations (sine and cosine) at every layer of a neural network. This design aims to embed the desirable properties of linear networks within a nonlinear framework. By doing so, it aims to leverage the consistent, plastic learning behavior of linear models while also providing the expressive power necessary for complex tasks. 

% However, while deep Fourier features have shown promise in continual learning, their fixed periodic functions may not perform optimally across diverse tasks, particularly in architectures where more common activation functions (e.g., ReLU, GELU) are used~\citep{radford2018improving,devlin2019bert}. This limitation underscores the need for further research into activation functions that can balance the preservation of plasticity with versatility across various neural network architectures and tasks.

In this work, we aim to provide a general approach for mitigating loss of plasticity that can be applied to any activation function. Our method is designed to avoid saturation effects while dynamically injecting linear components to sustain gradient flow and preserve plasticity. We describe our method in detail in the next section.



% Considering these methods, we propose an alternative perspective on why they help preserve plasticity: both approaches effectively \textit{cover} the saturation regions of activation functions. In deep Fourier features, the fixed periodic (sine and cosine) activations ensure that, even when one nonlinear component saturates, the other remains in a linear regime, thus preserving gradient flow. Similarly, CReLUs maintain activation diversity by duplicating responses with opposite signs, effectively ensuring that some portion of each neuron's output stays unsaturated. Motivated by this insight, we introduce an adaptive residual linearity injection mechanism where each neuron dynamically adjusts its linear contribution based on its own saturation state. This adaptive mechanism not only retains the benefits of covering the saturation domain—thereby maintaining plasticity—but also offers the flexibility to tailor the balance between linearity and nonlinearity to the specific demands of each task. In doing so, our method builds on the strengths of existing approaches while providing a more versatile framework for continual learning.




% Mention the next part somewhere else (may be in ablation for interpolation?)



% In addition to leveraging fixed deep Fourier features, the paper introduces the concept of α\alpha-linearization as a means to systematically blend linearity with nonlinearity within activation functions. Specifically,  α\alpha-linearization redefines an activation function ϕ\phi as
% \begin{equation}
% \phi_{\alpha}(x) = \alpha x + (1 - \alpha) \phi(x),
% \end{equation}
% where the parameter $\alpha$ governs the trade-off between purely linear behavior ($\alpha$ = 1) and the original nonlinear response ($\alpha$ = 0).
% This tunable interpolation not only enhances the \textit{unit sign entropy}—ensuring that activations remain balanced between positive and negative values—but also helps mitigate issues such as saturation and unit linearization that can impede continual learning. However, a critical challenge is the sensitivity of performance to the precise tuning of $\alpha$. Even with optimal tuning, a high $\alpha$ can result in overly linear representations that slow down training, while a low $\alpha$ may fail to adequately preserve plasticity.

% In this work, we aim to concentrate on this aspect and address the fixed $\alpha$
% issue. 








==> sections/3-problem_setting.tex <==
\section{Problem Setting}
\roozbeh{
In this paper, we focus on mitigating plasticity loss in continual supervised learning. Although much of the continual learning literature has traditionally concentrated on reducing catastrophic forgetting, recent studies have highlighted that plasticity loss becomes a critical issue, particularly when training spans long sequences of tasks. As an agent encounters a nonstationary data stream over its lifetime, the gradual loss of plasticity can significantly impair its ability to learn new tasks. Hence, our study is dedicated exclusively to addressing plasticity loss, setting aside the problem of catastrophic forgetting.


==> sections/4-toy_example.tex <==
\section{Motivating Example}

==> sections/6-Experimental_setup.tex <==
\section{Motivating Example}


\section{Introduction}

\khashi{
Continual learning studies how an agent adapts to a sequence of tasks while encountering an ever-changing distribution of new data. Unlike humans and other biological agents, which excel at lifelong learning, deep learning models struggle due to plasticity loss—a gradual decline in their ability to learn and adapt—especially in non-stationary data settings, where a model trained on one task finds it difficult to acquire new knowledge from subsequent tasks. 
% Recent research has attributed this phenomenon to factors such as growing parameter norms, increased linearization, and changes in the curvature of the loss landscape. 
To address this challenge, recent approaches have mostly focused on regularizing the network during training or periodically reinitializing a subset of weights to restore learning capacity. While these methods can alleviate plasticity loss in controlled benchmarks, they often come with
limitations—regularization can overly constrain the model, reducing its overall capacity and performance, while reinitialization, which often depends on explicit task boundaries, disrupts learned representations, making it less suitable for real-world applications where tasks evolve continuously.

Conversely, another line of research has focused on the influence of activation functions on plasticity loss in neural networks, highlighting their essential role in maintaining a model's learning ability over time. A simple example of this concept is illustrated in Figure \ref{fig:toy_example}, where different activation functions yield distinct outcomes on the Random-label MNIST task \footnote{}, with some effectively preventing plasticity loss. Notably, even in this simple example, standard activation functions like ReLU, GeLU, and Tanh fail to sustain the network’s learning capacity, experiencing significant degradation over time, while alternatives such as  CReLU and PReLU help maintain plasticity across tasks.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{figures/toy_example.png}
    \caption{The impact of different activation functions on plasticity loss in the Random-label MNIST task. Activation functions such as Cosine, CReLU, and PReLU help sustain the network’s learning capacity over multiple tasks, while others experience significant degradation. This highlights the crucial role of activation function choice in maintaining plasticity and long-term learning ability in neural networks.}
    \label{fig:toy_example}
\end{figure}

Moreover, recent theoretical studies  suggest that increased linearity in the learned function space represented by a neural network can make models more robust to plasticity loss. While non-linearity enables networks to capture complex representations, it can also impose constraints that hinder future learning. To address this trade-off, approaches like deep Fourier features use fixed sine and cosine activations to embed the behavior of deep linear networks, preserving high plasticity. Although deep Fourier features have shown promise in continual learning, they embed a deep linear model within the network by having each neuron output two components, one of which is always linear with respect to the input. 
In this work,  rather than maintaining a fixed proportion of linear components in the network, we propose a more effective approach that allows each neuron to adaptively determine the balance between linearity and non-linearity. This flexibility enables the model to \textit{adapt} its degree of linearity based on the specific demands of each task, potentially leading to better performance in continual learning scenarios. Figure ?? illustrates this characteristic.




%Interestingly, the success of the cosine activation function in preserving plasticity aligns with recent theoretical findings: as the degree of non-linearity in an activation function increases, the model becomes more susceptible to plasticity loss. To address this issue, recent work on deep Fourier features employs fixed sine and cosine activations to approximate the behavior of deep linear networks, thereby maintaining high plasticity.
%However, while Deep Fourier features have shown promise in continual learning, their fixed periodic functions may not perform optimally across diverse tasks—especially in architectures where ReLU is dominant. This limitation highlights the need for further research into activation functions that can balance plasticity preservation with versatility across various neural network architectures and tasks.




While conventional deep learning models use fixed, static activation functions throughout training, neuroscience research suggests that individual neurons adapt their non-linearity based on context.
Although artificial neural networks (ANNs) remain far less sophisticated than their biological counterparts, neuroscience-inspired AI algorithms have achieved great attention in deep learning. 
One key difference between biological neurons and artificial neurons lies in how their activation functions operate.  Studies show that biological neurons dynamically adjust their response profiles in response to contextual factors and neuromodulatory influences, meaning their activation functions can change over time depending on stimuli or learning conditions. This adaptability contrasts sharply with traditional deep learning architectures, where activation functions remain unchanged. The absence of such dynamic mechanisms in artificial neural networks may contribute to challenges in continual learning, particularly the loss of plasticity.



 Inspired by biological insights and the relationship between representation linearity and plasticity loss, we introduce \texttt{AdaLin}, a simple yet effective approach that allows each neuron to adaptively learn an \textit{interpolation parameter}, dynamically adjusting its activation function between linear and nonlinear components. Unlike heuristic-based methods, \texttt{AdaLin} enables the model to maintain plasticity naturally through gradient descent. This adaptability allows some neurons to modulate their linear component while others retain non-linearity, striking a balance between the stability of linear models and the expressive power of nonlinear activations.

We evaluate \texttt{AdaLin} on multiple continual learning benchmarks, demonstrating that it matches or outperforms recent methods without introducing additional hyperparameters or relying on task boundary information. Additionally, because each neuron's learned parameter is interpretable, we analyze these parameters across tasks to reveal the network’s tendency toward linear or nonlinear behavior. Our results show that in most tasks, only a small fraction of neurons adopt a linear response. Finally, we conduct extensive ablation studies, applying \texttt{AdaLin} to traditional activation functions and analyzing how various network properties evolve throughout training.
}
